Resource-Efficient Federated Fine-Tuning Large Language Models for Heterogeneous Data

Fine-tuning large language models (LLMs) via federated learning, i.e., FedLLM, has been proposed to adapt LLMs for various downstream applications in a privacy-preserving way. To reduce the fine-tuning costs on resource-constrained devices, FedLoRA is proposed to fine-tune only a small subset of model parameters by integrating low-rank adaptation (LoRA) into FedLLM. However, apart from resource constraints, there is still another critical challenge, i.e., data heterogeneity, severely hindering the implementation of FedLoRA in practical applications. Herein, inspired by the previous group-based federated learning paradigm, we propose a hierarchical FedLoRA framework, termed HierFedLoRA, to address these challenges. Specifically, HierFedLoRA partitions all devices into multiple near-IID groups and adjusts the intra-group aggregation frequency for each group to eliminate the negative effects of non-IID data. Meanwhile, to reduce the computation and communication cost, HierFedLoRA dynamically assigns diverse and suitable fine-tuning depth (i.e., the number of continuous fine-tuning layers from the output) for each group. HierFedLoRA explores jointly optimizing aggregation frequency and depth upon their coupled relationship to better enhance the performance of FedLoRA. Extensive experiments are conducted on a physical platform with 80 commercial devices. The results show that HierFedLoRA improves the final model accuracy by 1.6% to 4.2%, speeding up the fine-tuning process by at least 2.1$\times$, compared to the strong baselines.

==> contents/overview.tex <==
As illustrated in Figure \ref{framework}, \oursys consists of two key components with a total of six main modules, \ie, the PS with five modules and the device with one module.
The details of each module are as follows:

\textbf{Device Status Monitoring.}
The PS periodically collects information about the current working status of all devices (\eg, label distribution, computing, and communication capabilities) to make effective fine-tuning strategies. 

\textbf{Device Grouping.}
Based on the collected status information, the PS dynamically partitions the devices into proper groups using the proposed efficient grouping algorithm to promote system efficiency.

\textbf{Depth and Frequency Optimization.}
In this module, the PS simultaneously determines the appropriate fine-tuning depth and aggregation frequency for each group.

\textbf{Local Fine-Tuning}
The device fine-tunes the LLM by updating LoRA parameters, periodically uploading them to the PS for aggregation, and reporting status (\eg, computing and communication time) for strategy optimization.

\textbf{Group Aggregation.}
The module manages LoRA parameters for the groups, ensuring efficient organization and storage of updates, and performs group-level aggregation.

\textbf{Global Aggregation.}
This module performs global-level aggregation, combining LoRA parameters across groups to derive the global model parameters.

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\columnwidth]{figs/sys_design.pdf}
    \vspace{-0.2cm}
    \caption{The proposed framework \oursys.}
    \label{framework}
    \vspace{-0.5cm}
\end{figure}

==> contents/related_word.tex <==
% \textbf{Large language model.}
The development of modern natural language processing (NLP) traces back to the introduction of the transformer architecture by Vaswani \etal in 2017 \cite{vaswani2017attention}. 
Upon transformers, groundbreaking large language models (LLMs) such as BERT \cite{devlin2018bert}, GPT-2 \cite{radford2019language}, and more recently LLaMA \cite{touvron2023llama} have achieved state-of-the-art results across various NLP tasks. 
The LMs are first pre-trained on the vast corpus to learn general features and patterns and then fine-tuned on task-specific datasets to adapt downstream applications \cite{cai2022fedadapter}. 
However, due to data privacy, it is impractical to collect enough data from the devices for centralized fine-tuning \cite{mcmahan2017communication, lin2021fednlp}, and thus federated fine-tuning LLMs, called FedLLM, becomes the evolution direction.

% FedLLM (\eg, FedNLP \cite{lin2021fednlp}) enables multiple devices to collaboratively fine-tune LMs for various domains but faces the challenges of resource constraints and data heterogeneity. 
To reduce the heavy resource cost on the device, modern FedLLM utilizes parameter-efficient fine-tuning methods (PEFT), such as Adapter \cite{houlsby2019parameter} and LoRA \cite{hu2021lora}, due to the limited on-device resources. 
PEFT methods freeze most LLM parameters and only fine-tune additional lightweight parameters (typically less than 1\%).
Due to its superior performance and computational efficiency, LoRA has become one of the most widely adopted methods in FedLLM (FedLoRA).
Early works mainly focus on improving LoRA initialization to address data heterogeneity.
For example, %Babakniya \etal \cite{babakniya2023slora} propose 
SLoRA \cite{babakniya2023slora} begins with full fine-tuning of the original LLM, followed by singular value decomposition (SVD) to decompose gradient updates for LoRA initialization. 
Besides, FedDeRA \cite{yan2024federa} is developed to directly apply SVD on pre-trained weights for LoRA initialization.
Although LoRA initialization is easy to deploy, it often results in degraded performance, especially in heterogeneous data scenarios where parameter drift contributes to degradation. 
In addition, some works improve the performance of FedLoRA by adjusting LoRA ranks for devices. 
For instance, Cho \etal \cite{cho2023heterogeneous} introduce HetLoRA, which assigns appropriate ranks to devices and aggregates heterogeneous LoRA parameters via zero-padding. 
Building upon this, Bai \etal \cite{bai2024federated} present FlexLoRA, a method that employs a dynamic parameter allocation strategy to adjust LoRA rank and utilizes SVD for weight redistribution.
While rank optimization is straightforward and reduces communication overhead to some extent, it fails to lower the computational overhead.
This is because updating even a small number of LoRA parameters requires full forward and backward propagation, resulting in computational costs comparable to full fine-tuning. 

% For example, Zhang \etal \cite{zhang2023fedpetuning} first validate the effectiveness of Adapter in FedLLM, and Cai \etal \cite{cai2022fedadapter} propose FedAdapter to improve the efficiency of Adapter-based FedLLM approach. 
% However, Adapter inevitably bring additional inference latency, potentially resulting in up to 30\% latency \cite{hu2021lora}. 
% To avoid the inference latency and explore the potential of LoRA in FedLLM, Zhang \etal \cite{zhang2023fedpetuning} propose FedLoRA and verify the efficiency of LoRA in the context of FedLLM through extensive experiments.
% Upon FedLoRA, Cho \etal \cite{cho2023heterogeneous} propose HetLoRA, in which each device adds LoRA layers to all transformer layers with a diverse and appropriate LoRA rank to deal with system heterogeneity.
% However, due to the rank mismatch of all LoRA layers on different devices, it is difficult to aggregate these layers, resulting in poor fine-tuning performance.
% In conclusion, existing works simply add LoRA layers with the uniform rank distribution for all transformer layers, which still requires substantial computing and communication resources, resulting in slow fine-tuning speeds.
% Besides, system heterogeneity further leads to low training efficiency or poor fine-tuning performance \cite{kim2021autofl, luo2022tackling, liao2023mergesfl}.
% In other words, in the context of FedLLM, existing works still face significant limitations, as they fail to achieve both high accuracy and fast convergence.
% This is especially evident with resource-constrained and heterogeneous devices, where these methods fail to effectively address the above challenges.
% On the contrary, LEGEND assigns diverse and suitable LoRA depths for heterogeneous devices to improve fine-tuning efficiency, while generating reasonable rank distribution to further enhance performance. 
% Thus, LEGEND effectively addresses the aforementioned challenges while saving computing and communication costs.



